The VMC Survey -- XLIX. Discovery of a population of quasars dominated by nuclear dust emission behind the Magellanic Clouds

Following the discovery of SAGE0536AGN ($z \sim$ 0.14), with the strongest 10-$\mu$m silicate emission ever observed for an Active Galactic Nucleus (AGN), we discovered SAGE0534AGN ($z \sim$ 1.01), a similar AGN but with less extreme silicate emission. Both were originally mistaken as evolved stars in the Magellanic Clouds. Lack of far-infrared emission, and therefore star-formation, implies we are seeing the central engine of the AGN without contribution from the host galaxy. They could be a key link in galaxy evolution. We used a dimensionality reduction algorithm, t-SNE (t-distributed Stochastic Neighbourhood Embedding) with multi-wavelength data from Gaia EDR3, VISTA survey of the Magellanic Clouds, AllWISE and the Australian SKA Pathfinder to find these two unusual AGN are grouped with 16 other objects separated from the rest, suggesting a rare class. Our spectroscopy at SAAO/SALT and literature data confirm at least 14 of these objects are extragalactic ($0.13 < z < 1.23$), all hosting AGN. Using spectral energy distribution fitter CIGALE we find that the majority of dust emission ($> 70 \%$) in these sources is due to the AGN. Host galaxies appear to be either in or transitioning into the green valley. There is a trend of a thinning torus, increasing X-ray luminosity and decreasing Eddington ratio as the AGN transition through the green valley, implying that as the accretion supply depletes, the torus depletes and the column density reduces. Also, the near-infrared variability amplitude of these sources correlates with attenuation by the torus, implying the torus plays a role in the variability.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
